Reducing Data Fragmentation in Data Deduplication Systems via Partial Repetition and Coding

Data deduplication, one of the key features of modern Big Data storage devices, is the process of removing replicas of data chunks stored by different users. Despite the importance of deduplication, several drawbacks of the method, such as storage robustness and file fragmentation, have not been previously analyzed from a theoretical point of view. Storage robustness pertains to ensuring that deduplicated data can be used to reconstruct the original files without service disruptions and data loss. Fragmentation pertains to the problems of placing deduplicated data chunks of different user files in a proximity-preserving linear order, since neighboring chunks of the same file may be stored in sectors far apart on the server. This work proposes a new theoretical model for data fragmentation and introduces novel graph- and coding-theoretic approaches for reducing fragmentation via limited duplication (repetition coding) and coded deduplication (e.g., linear coding). In addition to alleviating issues with fragmentation, limited duplication and coded deduplication can also serve the dual purpose of increasing the robusteness of the system design. The contributions of our work are three-fold. First, we describe a new model for file structures in the form of self-avoiding (simple) paths in specialized graphs. Second, we introduce several new metrics for measuring the fragmentation level in deduplication systems on graph-structured files, including the stretch metric that captures the worst-case "spread" of adjacent data chunks within a file when deduplicated and placed on the server; and, the jump metric that captures the worst-case number of times during the reconstruction process of a file that one has to change the readout location on the server. For the stretch metric, we establish a connection between the level of fragmentation and the bandwidth of the file-graph. In particular, ...

==> abstract.tex <==

\begin{abstract}
Motivated by testing for pathogenic diseases we consider a new nonadaptive group testing problem for which: (1) positives occur within a burst, capturing the fact that infected test subjects often come in clusters, and (2) that the test outcomes arise from semiquantitative measurements that provide coarse information about the number of positives in any tested group.
% Motivated by group testing applications 
% in genotyping, and in particular, 
% such as COVID-19 testing, where positive cases tend to occur in bursts, we consider the problem of identifying 
% we address the problem of
% identifying a single burst of positive (infected) individuals in a pool of linearly ordered test samples using non-adaptive semiquantitative measurements. 
{Our model generalizes prior work on detecting a single burst with classical group testing~\cite{colbourn1999} to the setting of semiquantitative group testing (SQGT)~\cite{emad2014semiquantitative}.}
% which has until now not addressed the issue of bursty positives.
Specifically, we study the setting where the burst-length $\ell$ is known and the semiquantitative tests provide potentially nonuniform estimates on the number of positives in a test group. The estimates represent the index of a quantization bin containing the (exact) total number of positives, for arbitrary thresholds $\eta_1,\dots,\eta_s$. Interestingly, we show that the minimum number of tests needed for burst identification is essentially only a function of the largest threshold $\eta_s$. In this context, our main result is an order-optimal test scheme that can recover any burst of length $\ell$ using roughly {$\lfloor\frac{\ell}{2\threshold{s}}\rfloor+\log_{s+1}(n)$} measurements. 
This suggests that a large saturation level $\eta_s$ is more important than finely quantized information when dealing with bursts. We also provide results for related modeling assumptions and specialized choices of thresholds. 
% Additionally, we provide extensions to the case where only an upper bound on the burst length is known.
% When the burst length is known to be $\ell$, we give an optimal scheme for any SQGT quantized thresholds satisfied $l\geq \threshold{s}\log_{2}(\threshold{s})$ with $\approx\frac{l}{2\threshold{s}}+\log_{s+1}(n)$ tests. Surprisingly, there is no loss to only use the single biggest threshold $\threshold{s}$ when $l=\omega\lp\threshold{s}\log_{2}(n)\rp$. When the upper bound of burst length is known ($\leq l$), we give an optimal scheme for Saturated SQGT quantized thresholds with $\approx\frac{l}{\threshold{s}}+\log_{2}(n)$ tests.
\end{abstract}

==> almost_line.tex <==
\begin{IEEEproof}
    Pick any starting point $v\in V$, then $s= N(v, 0, G),N(v, 1, G),\hdots$ would be a linerization with edge stretch $\leq 4|E_{arch}|+2$, where elements in the same $N(v, i, G)$ can be placed in any order. Because each edge is either within the same $N(v, i, G)$ or between $N(v, i, G)$ and $N(v, i+1, G)$. Therefore $B(G)\leq 2\max_{i}|N(v, i, G)|$. It remains to show $\max_{i}|N(v, i, G)|\leq 2|E_{arch}|+1$  
\end{IEEEproof}

==> sec_limits.tex <==
%\subsection{Fundamental limits for the non-adaptive case}
We first provide lower bounds for the smallest number of measurements needed for the $\mini{\Burstfx}$ and $\mini{\Burstbnd}$ settings. The proofs mostly use ideas from~\cite{colbourn1999}.
\begin{theorem}\label{LB_fix}\label{LB_variable} We have
    \begin{equation*}
        \begin{cases}
        \mini{\Burstfx}\geq \max\lp\log_{s+1}\lp n-\ell+1\rp,\lceil\frac{\ell}{2\threshold{s}}\rceil\rp,\\
        \mini{\Burstbnd}\geq \max\lp\log_{2}\lp n\rp,\lceil\frac{\ell}{s}\rceil\rp.
        \end{cases}   
    \end{equation*}
\end{theorem}

The proof technique used for $\mini{\Burstbnd}$ is similar to that for $\mini{\Burstfx}$; hence, we only provide the proof for $\mini{\Burstfx}$.   
We prove the first bound by establishing each of the bounds on the right-hand side separately and combining them via maximization. 
\begin{enumerate}
    \item The bound $\log_{s+1}\lp n-\ell+1\rp$ follows from a simple counting argument: there are a total of $n-\ell+1$ different head positions and a total of $s+1$ possible outcomes for each measurement.
    \item The bound $\lceil\frac{\ell}{2\threshold{s}}\rceil$: we show that even if we only require to discriminate among the first $\ell+1$ bursts (i.e., bursts $\burstwh{b}{i}$ with $0\leq i\leq\ell$), we still need $\lceil\frac{\ell}{2\threshold{s}}\rceil$ measurements. For any measurement $\bm{m}$, let $\bm{m}_{1}$ and $\bm{m}_{2}$ denote the first and second block of $\ell$ bits of $\bm{m}$. Only the last $\threshold{s}$ nonzero bits in $\bm{m}_{1}$ and the first $\threshold{s}$ nonzero bits in $\bm{m}_{2}$ are relevant. For simplicity, we only provide a proof for the $\bm{m}_{2}$ case. Let $\ell\leq i_{1}<i_{2}<\hdots<2\ell$ be the elements included in $\bm{m}_{2}$. Since $\length{b}=\ell$ and $\head{b}\leq\ell$, if $i_{j}$ is included in the burst $\burst{b}$ then $i_{1},\hdots,i_{j-1}$ must also be included. Therefore, if $j>\threshold{s}$, by observing that $\threshold{s}$ is the largest threshold, one can remove $i_{j}$ from $\bm{m}_{2}$ without changing the outcome. Hence one can only retain the first $\threshold{s}$ nonzero bits in $\bm{m}_{2}$ and still arrive at the same outcome. As a result, it suffices to only consider those $\bm{m}$ for which $\sum_{j=0}^{2\ell-1}\bm{m}(j)\leq 2\threshold{s}$. Let $\mb{M}^{h_{\mb{M}}\times 2\ell}$ be our measurement matrix restricted to the first $2\ell$ columns. Suppose that $h_{\mb{M}}<\frac{\ell}{2\threshold{s}}$; then $\sum_{i=0}^{h_{\mb{M}}-1}\sum_{j=0}^{2\ell-1} \mb{M}(i,j)\leq 2\threshold{s}h_{\mb{M}}<\ell$. This implies that there exists a $0\leq j<\ell$ such that $\mb{M}(*,j)=\mb{M}(*,j+\ell)=\bm{0}^{\height{\mb{M}}\times 1}$. Then $\thresholds\lp\mb{M}\burstwh{b}{i+1}\rp= \thresholds\lp\mb{M}\burstwh{b}{i}+\mb{M}(*,j+\ell)-\mb{M}(*,j)\rp=\thresholds\lp\mb{M}\burstwh{b}{i}\rp$. Therefore $\mini{\Burstfx}\geq \lceil\frac{\ell}{2\threshold{s}}\rceil$. 
\end{enumerate}









==> sec_relatedwork.tex <==
The problem is closely related to the extensively studied `bandwidth problem' for graphs~\cite{diaz2002survey,petit2013addenda}:
%\begin{problem}
    Given a graph $G=(V,E)$, find a permutation $\sigma^{*}$ over $\mathbb{S}_n,$ the symmetric group of order $n$ that minimizes the worst-case edge stretch, $B(G):=\min_{\sigma}\max_{uv\in E}|\sigma(u)-\sigma(v)|.$
%\end{problem}
The graph bandwidth problem is NP-hard for general graphs. It is also NP-hard for trees with maximum degree $3$ and other subclasses of graphs~\cite{petit2013addenda}. The best known results for general graphs with efficient placement algorithms give an   approximation ratio of $O(\log^{3}(n)\sqrt{\log\log(n)})$ \cite{dunagan2001euclidean}. On the other hand, achieving an approximate within any constant $k\in N$ is NP-hard~\cite{unger1998complexity}. Still, for certain subclasses of graphs, more precise results can be derived. 

More specifically, the graph linearization and graph bandwidth problem are related as follows. Since the server chunk store  $s\in V^{n}$ is a permutation of $n$ chunks, $\forall w\in W(G,\leq t)$ we have $$\frac{\MinS(s,w)}{1+\ell(w)}\leq \frac{1+\sum_{i=1}^{\ell(w)}|s(w_{i})-s(w_{i+1})|}{1+\ell(w)}\leq \frac{1+\ell(w)B(G)}{1+\ell(w)}.$$ 
Furthermore, by the definition of the bandwidth, there exists $uv\in E$ such that $|s^{-1}(u)-s^{-1}(v)|\geq B(G)$. Together, these results imply that $\frac{B(G)}{2} \leq F_t(G,n) < B(G).$ In words, the bandwidth of a graph is an upper bound on the fragmentation level. Note that computing the bandwidth $B(G)$ for arbitrary graphs is computationally challenging, and existing general lower/upper bounds on $B(G)$ are mostly loose. This is why in the next section we turn our attention to a review of results from the graph bandwidth literature and subsequently focus on sparse Hamiltonian path graphs. The connection between the two problems for the case of a redundant chunk store is discussed in Section IV. Besides graph bandwidth, our problem is also related to a couple of graph optimization problems such as graph edgesum, profile width, pathwidth, cutwidth, cop and robber game, etc. Readers are referred to \cite{lai1999survey} for a comprehensive survey.
%\textcolor{red}{With the above definitions in place, we next turn our attention on providing bounds on the fragmentation level that do not rely on bandwidth results.} 
%For no redundancy, every vertex showed up exactly once (therefore $m=|V|$) in Problem~\ref{original_problem}, it's equivalent to finding the best permutation $\sigma$ over $V$ that minimizes the worst edge stretch.
%\begin{problem}[special case $m=|V|$]\label{bandwidth_problem}
%    Given a graph $G=(V,E)$, find $\sigma^{*}$ that achieve
%    \begin{equation*}
%        B(G):=\min_{\sigma}\max_{uv\in E}|\sigma(u)-\sigma(v)|
%    \end{equation*}
%\end{problem}    
%This problem is NP-hard for general graphs. Even remain NP-hard for trees with a maximum degree of $3$. 
%\iscomment{I think readers will find it a bit confusing that we introduce the fragmentation notion $F$, but then present most results in terms of $B(G)$. Would it be better to write $F_t(G,n)$ for the fragmentation level with files $W(G\leq t)$ and then use $F_2(G,n)$ instead of $B(G)$ (with the appropriate rescaling)?}
